AMECOS: A Modular Event-based Framework for Concurrent Object Specification

In this work, we introduce a modular framework for specifying distributed systems that we call AMECOS. Specifically, our framework departs from the traditional use of sequential specification, which presents limitations both on the specification expressiveness and implementation efficiency of inherently concurrent objects, as documented by Casta\~neda, Rajsbaum and Raynal in CACM 2023. Our framework focuses on the interactions between the various system components, specified as concurrent objects. Interactions are described with sequences of object events. This provides a modular way of specifying distributed systems and separates legality (object semantics) from other issues, such as consistency. We demonstrate the usability of our framework by (i) specifying various well-known concurrent objects, such as registers, shared memory, message-passing, reliable broadcast, and consensus, (ii) providing hierarchies of ordering semantics (namely, consistency hierarchy, memory hierarchy, and reliable broadcast hierarchy), and (iii) presenting a novel axiomatic proof of the impossibility of the well-known Consensus problem.

==> Paragraph/AsynchronyProof/Illustration-Asynch-Media.tex <==
\section{Illustrations of Asynchronous Communication Media}
\label{sec:examples-state-graphs}

In this section, we give some examples of distributed systems in which processes communicate using asynchronous communication objects, namely atomic shared memory and message-passing (reliable broadcast).
We observe that these examples satisfy the \Asynchrony property defined in \Cref{def:asynch-short}.
Then, we present two systems with objects that do not satisfy \Asynchrony, namely Test\&Set and total-order reliable broadcast.  



\begin{algorithm}[t]
\begin{algorithmic}
\State Process 1: $M.\wwrite(1, x)$
\State Process 2: $M.\wwrite(2, x)$
\State Process 3: $v \leftarrow M.\rread(x)$
\end{algorithmic}
\caption{Distributed system with 3 processes that write and read in a shared atomic register $x$.}
\label{alg:shared memory}
\end{algorithm}

\begin{figure}[t]
    \centering
    \rotatebox{0}{
        \includegraphics[width=0.98\textwidth]{fig/pdfPic/SharedMemory.pdf}
    }
    \caption{Set of states $S$ as a \emph{state graph} obtained from the histories of the system in \Cref{alg:shared memory}. Each node (box) is a state. A directed arrow labeled with an event $e$ between two states indicates a transition triggered by $e$ (see the $\Continuity(S)$ property). Events are abbreviated for clarity from their formal definition in \Cref{sec:shared-mem}: $\mathit{WI}_i(v)$, $\mathit{WR}_i$, $\mathit{RI}_i$ and $\mathit{RR}_i(v)$ are short for $M.\wwrite_i(v,x).\inv$, $M.\wwrite_i(v,x).\res$, $M.\rread_i(x).\inv$ and $M.\rread_i(x)/v.\res$, respectively. 
    The event indices are omitted for clarity. 
    }
    \label{fig:async-atomic-mem}
\end{figure}

The first example is an atomic register $x$ in a shared memory $M$.
\Cref{alg:shared memory} presents the algorithm executed by a distributed system formed by 3 processes, in which two of them write in $x$ while the third one reads from $x$.
\Cref{fig:async-atomic-mem} presents the set of states $S$ obtained from all the possible histories of the system of \Cref{alg:shared memory} as described in \Cref{sec:asynconcsystem}.
Observe in \Cref{fig:async-atomic-mem} that states do not contain information about how the two write operations in Processes 1 and 2 are ordered in real time.
The set is presented as a directed acyclic graph (DAG) with a single source node $\varnothing$, and a directed link labeled with event $e$ from a state $R$ to state $R \cup \{e\}$. This DAG has no cycles and \Continuity guarantees that it is connected. By inspection, it is possible to observe in \Cref{fig:async-atomic-mem} that the set $S$ satisfies \Asynchrony as defined in \Cref{def:asynch-short}.
%: For each state $R \in S$, if $R \cup \{e\} \in S$, $R \cup \{e'\} \in S$, and $e.\proc \neq e'.\proc$, then $R \cup \{e, e'\} \in S$. \nn{[CG+NN: This is the older definition of Asynchrony.]}

\begin{algorithm}[t]
\begin{algorithmic}
\State Process 1: $M.\wwrite(1, x)$; $v_1 \leftarrow M.\rread(x)$
\State Process 2: $M.\wwrite(2, x)$; $v_2 \leftarrow M.\rread(x)$
\end{algorithmic}
\caption{Distributed system with 2 processes that write and read in a shared atomic register~$x$.}
\label{alg:shared memory2}
\end{algorithm}

\begin{figure}[t]
    \centering
    \rotatebox{0}{
        \includegraphics[width=0.98\textwidth]{fig/pdfPic/SharedMemoryV2.pdf}
    }
    \caption{Set of states $S$ as a \emph{state graph} obtained from the histories of the system in \Cref{alg:shared memory2}. Events are abbreviated for clarity from their formal definition in \Cref{sec:shared-mem}: $\mathit{WI}_i(v)$, $\mathit{WR}_i$, $\mathit{RI}_i$ and $\mathit{RR}_i(v)$ are short for $M.\wwrite_i(v,x).\inv$, $M.\wwrite_i(v,x).\res$, $M.\rread_i(x).\inv$ and $M.\rread_i(x)/v.\res$, respectively. 
    The event indices are omitted for clarity. 
    }
    \label{fig:async-atomic-mem2}
\end{figure}

The second example also has an atomic register $x$ in a shared memory $M$.
\Cref{alg:shared memory2} presents the algorithm executed by a distributed system formed by 2 processes, in which both of them write in $x$ and then read from $x$.
\Cref{fig:async-atomic-mem2} presents the set of states $S$ obtained from all the possible histories of the system of \Cref{alg:shared memory2} as described in \Cref{sec:asynconcsystem}.
Observe again that in this figure states do not contain information about how the two write operations in Processes 1 and 2 are ordered in real time. For this reason in the last layer from each state there are two arrows labelled with the two possible different values read. By inspection, it can be observed that the set $S$ of \Cref{fig:async-atomic-mem2} satisfies \Asynchrony as defined in \Cref{def:asynch-short}.

\begin{algorithm}[t]
\begin{algorithmic}
\State Process 1: $v_1 \leftarrow T.\testandset()$
\State Process 2: $v_2 \leftarrow T.\testandset()$
\end{algorithmic}
\caption{Distributed system with 2 processes that use a Test\&Set object $T$ to coordinate.}
\label{alg:testandset}
\end{algorithm}

\begin{figure}[t]
    \centering
    \rotatebox{0}{
        \includegraphics[width=0.98\textwidth]{fig/pdfPic/TestAndSet.pdf}
    }
    \caption{Set of states $S$ as a \emph{state graph} obtained from the histories of the system in \Cref{alg:testandset}. Events are abbreviated for clarity: $\mathit{T\&SI}_i$ and $\mathit{T\&SR}_i(v)$ are short for $T.\testandset_i().\inv$ and $T.\testandset_i()/v.\res$, respectively.
    The event indices are omitted for clarity.}
    \label{fig:async-testAndSet}
\end{figure}

For comparison, we present in \Cref{alg:testandset} the algorithm run by a system with two processes that use a Test\&Set object $T$ \cite{FIS64,R13}. This object has an operation \testandset that returns a value $0$ the ``first'' time it is invoked and a value $1$ in any invocation after that. \Cref{fig:async-testAndSet} shows the set $S$ as a DAG obtained from all the histories of this system. It can be observed that $S$ does not satisfy \Asynchrony, since it is violated for state $R=\{\mathit{T\&SI}_1, \mathit{T\&SI}_2\}$ and events
$e=\mathit{T\&SR}_1(0)$ and $e'=\mathit{T\&SR}_2(0)$ (using the notation of the figure). Observe that the object $T$ could be used to solve consensus among the 2 processes, since the consensus number of Test\&Set is 2 \cite{H91,R13}.

\begin{algorithm}[t]
\begin{algorithmic}
\State Process 1: $B.\rbroadcast(m_1, 1)$
\State Process 2: $B.\rbroadcast(m_2, 2)$
\end{algorithmic}
\caption{Distributed system with 2 processes that use a reliable broadcast object $B$ to send 2 messages $m_1$ and $m_2$.}
\label{alg:rbcast}
\end{algorithm}

\begin{figure}[t]
    \centering
    \rotatebox{0}{
        \includegraphics[width=0.98\textwidth]{fig/pdfPic/BroadcastRegular.pdf}
    }
    \caption{Set of states $S$ as a \emph{state graph} obtained from the histories of the system in \Cref{alg:rbcast}. Events are abbreviated for clarity: $\mathit{B}_i(m_i)$ and $\mathit{D}_i(m_j)$ are short for $B.\rbroadcast_i(m_i, i).\inv$ and $B.\rdeliver_i/(M_j, j, j).\res$, respectively. The states in which a process receives a message before invoking \rbroadcast, the $B.\rbroadcast_i(m_i, i).\res$ events, and the event indices are omitted for clarity.}
    \label{fig:async-Broadcast-Normal}
\end{figure}

The third example we present is a system with two processes that use a reliable broadcast object $B$ to send respective messages $m_1$ and $m_2$, as presented in \Cref{alg:rbcast}.
\Cref{fig:async-Broadcast-Normal} presents a subset of the set $S$ obtained from the histories of this system.
For clarity, we have omitted the response events of the \rbroadcast op-exes, the states in which a process receives a message before invoking its local \rbroadcast op-ex, and the event indices. Observe that the four sink states only differ in the order in which they receive the messages (captured by the indices of the \rdeliver events). It can also be observed that \Asynchrony is satisfied.

\begin{algorithm}[t]
\begin{algorithmic}
\State Process 1: $B.\tobroadcast(m_1, 1)$
\State Process 2: $B.\tobroadcast(m_2, 2)$
\end{algorithmic}
\caption{Distributed system with 2 processes that use a total-order reliable broadcast object $B$ to send 2 messages $m_1$ and $m_2$.}
\label{alg:tobcast}
\end{algorithm}

\begin{figure}[t]
    \centering
    \rotatebox{0}{
        \includegraphics[width=0.98\textwidth]{fig/pdfPic/BroadcastTO.pdf}
    }
    \caption{Set of states $S$ as a \emph{state graph} obtained from the histories of the system in \Cref{alg:tobcast}. Events are abbreviated for clarity: $\mathit{TB}_i(m_i)$ and $\mathit{TD}_i(m_j)$ are short for $B.\tobroadcast_i(m_i, i).\inv$ and $B.\todeliver_i/(M_j, j, j).\res$, respectively. 
    The states in which a process receives a message before invoking \tobroadcast, the $B.\tobroadcast_i(m_i, i).\res$ events, and the event indices are omitted for clarity.}
    \label{fig:async-broadcast-TO}
\end{figure}

Finally, we present a system with a similar message-passing algorithm, presented in \Cref{alg:tobcast}, but that in this case uses a total order reliable broadcast object $B$ instead of simply \rbroadcast.
\Cref{fig:async-broadcast-TO} shows a subset of the set $S$, in which some states and events are omitted as before for clarity.
However, it can be seen in the resulting DAG that now only 2 sink states exist since both processes receive the messages in the same order.
This prevents the \Asynchrony axiom from being satisfied.

==> Paragraph/Consensus-Proof-short.tex <==
\section{Asynchronous Resilient Consensus Impossibility}
\label{sec:consensus-sketch}

This section further exemplifies the framework's utility by showing how it can be used to construct axiomatic proofs.
Particularly, we demonstrate the FLP impossibility of having consensus in an asynchronous system with process failures~\cite{FLP85}.
Due to page limitation, we provide a high-level overview of the proof in this section, but the full developments can be found in \Cref{sec:consensus}.

\paragraph{The Consensus object.}
Without loss of generality, we consider a simplified version of the consensus object $\Consensus$, which only has one notification operation, $\Consensus.\decide_i(v)$, returning a value $v \in V$ (we have binary consensus if $V = \{0,1\}$) to process $p_i$.
{\em Proving the impossibility of this weaker version makes our proof more general.}
We give in the following the semantics of the \decide notification operation.
If $o \equiv \Consensus.\decide_i/v$, then we have the following predicates.
\begin{align*}
    \decide.\safep(o,(O_c,\oo_c)) &\triangleq (v \in V)
    %&
    %\land (\Nexists \Consensus.\decide_i(-) \in O_c) 
    %&
    \land (\Forall \Consensus.\decide_j/v' \in O_c: v=v'). \\
    %
    \decide.\livep(o,H,\oo) &\triangleq \Exists \Consensus.\decide_j/- \in O.
\end{align*}
The \safep predicate states that the values decided are in the appropriate set $V$ and that, in the context of each op-ex, 
%no process decides more than once, and 
all decided values are the same.
Observe that we allow the same process to decide several times as long as the decided values are the same.
The \livep predicate states that some process must decide. 
% in every history.

\paragraph{Set of states of the system ($\bm{\Sigma}$).}
% \paragraph{Set of states of the system (\States).}
In the proof, we consider a system with a consensus object $\Consensus$ and a communication medium object $M$. We use the (potentially infinite) set $\Histories$ to capture all the histories of the system executions. \jw{From each execution, a history is obtained that contains only the events of objects $\Consensus$ and $M$ in the order they occurred.} From these histories, we will construct a (potentially infinite) set $\States$ of possible states of the system.
Each \emph{state} $\state \in \States$ is a (potentially infinite) set of events.
Intuitively, a state $\state$ is the collection of local states of all system processes $p_i$, represented by the totally-ordered local events that $p_i$ has experienced.
We also assign an \emph{index} to each event in a history $H=(E,\eo,O,P) \in \Histories$.
The index assigned to event $e \in E$ is an attribute $e.\idx$ that is the position of $e$ in the sequence of events of its process $e.\proc$.
This sequence is obtained by ordering with $\eo$ the set $E|e.\proc$.

A special subset of $\States$ is the set of \emph{complete states}, defined as 
    $\complete(\States) \triangleq \{E \mid (E,\eo,O,P) \in \Histories \}.$
Consider now any history $H=(E,\eo,O,P) \in \Histories$.
We say that state $\state = E \in \complete(\States) \subseteq \States$ is a \emph{state extracted from $H$.}

\paragraph{The $\bm{\mathit{Continuity}}$ property.}
% \paragraph{The \Continuity property.}
% Observe that this construction of the set $\States$ guarantees the \Continuity property, which states that, from each nonempty state, we can always remove an event to get a substate.
\ta{This property ensures that, from every nonempty state $\state \in \States$, a previous substate $\state' = \state \setminus \{e\}$ can be obtained by removing one event $e$ using the following recursive procedure exhaustively.}
% We apply \ta{recursively} and exhaustively the following procedure to add more states to $\States$:
If $\state \in \States$ is a state extracted from $H$, let $e$ be the event in $\state$ with the largest index $e.\idx$ of those from process $e.\proc$,
then $\state' = \state \setminus \{e\}$ is also \emph{a state in $\States$ extracted from $H$.}
This procedure ends when the empty state $\varnothing$ is reached (which is also in $\States$).
%
Hence, $\States$ contains a state $\state$ iff there is a history $H=(E,\eo,O,P) \in \Histories$ such that the events in $\state$ from every process $p \in P$ are a prefix of the sequence of all events from $p$ in $E$ ordered by $\eo$.

\paragraph{The $\bm{\mathit{Asynchrony}}$ axiom.}
% \paragraph{The \Asynchrony axiom.}
An asynchronous system's set of states $\States$ must satisfy the \Asynchrony axiom, which requires that, if two states differ only in their last respective events, which are from different processes, their union is also a state. Observe that this must hold even if the two states are extracted from different histories.
%
We point out that our impossibility proof is agnostic of the communication medium object $M$, as long as the medium satisfies asynchrony as defined above.
\af{For completeness we show in \Cref{sec:asych-axiom-register-channel} that atomic registers and message-passing objects satisfy this axiom.}

\paragraph{The $\bm{\mathit{Val}}$ function.}
% \paragraph{The \valence function.}
Our impossibility proof relies on the notion of \emph{valence}, which was first introduced in~\cite{FLP85}.
We represent it as a function $\valence(\state)$, taking a state $\state$ as a parameter, and returning the set of all possible decision values that can be reached from this state (by extending $\state$ with more events, or because $\state$ already contains some \decide events). 
%\TA{Maybe we should express the first point formally}
% \JW{DELETE:Intuitively, }
% The valence of a complete state is the set of all values that were decided in the histories from which it was extracted, and, by \Branching, the valence of an incomplete state is the union of the valences of all \jw{the states obtained by adding one event to it}.
The valence of a complete state is the set of all values that were decided in the histories from which it was extracted.
\ta{Moreover, the valence of an incomplete state is the union of the valences of all \jw{the states obtained by adding one event to it}.
We call this last property \Branching.}
We say that a state $\state \in \States$ is \emph{univalent} iff we have $|\valence(\state)|=1$, and we say that it is \emph{multivalent} iff we have $|\valence(\state)|>1$.

\paragraph{The $\bm{\mathit{NonEmptyValence}}$ lemma.}
% \paragraph{The \PositiveValence lemma.}
\jw{This lemma uses the \livep predicate of the \Consensus object to show that there is no state $\state$ with an empty valence, $|\valence(\state)|=0$ (proof in \Cref{sec:consensus}).}

\paragraph{The $\bm{\mathit{Termination}}$ lemma.}
% \paragraph{The \Termination lemma.}
\ta{This lemma shows} that all complete states have a finite univalent sub-state (proof in \Cref{sec:consensus}).

\paragraph{The $\bm{\mathit{Resilience}}$ axiom.}
% \paragraph{The \Resilience axiom.}
This axiom states that, for any process, any multivalent state can be extended by an event that is not from this process.
This ensures that even if one process stops taking steps (\ie crashes), the system can still progress and reach a decision.

\paragraph{The $\bm{\mathit{NonTriviality}}$ axiom.}
% \paragraph{The \NonTriviality axiom.}
This axiom states that there exist 2 states with different valences, implying that there are histories deciding different values.

\paragraph{The impossibility theorem.}
The proof of the impossibility of asynchronous resilient consensus consists in showing that a contradiction lies in the system of axioms that we have created.
Firstly, we show that \NonTriviality, \Continuity, and \Branching imply the existence of a multivalent state.
From this multivalent state and using \Termination, we can find a \emph{critical} state, \ie a multivalent state for which all extensions are univalent.
By \Branching from the critical state, we can find two univalent 1-event extensions with different valences.
Let us consider the two distinct events, $e$ and $e'$, that extend the critical state into these two superstates with different valences.
If $e.\proc \neq e'.\proc$, then \Asynchrony applies, and we can create an extension of the critical state containing both $e$ and $e'$, however, by \Branching and \PositiveValence, this state would be multivalent, which contradicts the definition of a critical state.
Otherwise, if $e.\proc=e'.\proc$, then by \Resilience, we can create another 1-event extension of the critical state, whose valence is different from at least one of the two previous extensions (that of $e$ or that of $e'$).
This makes us fall back to the case $e.\proc \neq e'.\proc$, again yielding a contradiction.
Therefore, in all cases, the system of axioms leads to a contradiction.
(The details of the proof can be found in \Cref{sec:consensus}).

==> Paragraph/Constrains.tex <==
\section{Constraints}
\label{sec:Constraints}

% It is possible to formally define these constraints on the UML model using OCL (\textit{Object Constraint Language}), a language tailored for adding constraints to UML models.
% We first provide predicates defining strict order relations as follows.

% \begin{definition}[Generic strict orders]
% \label{def:generic-orders}
% Given an arbitrary set $S$ and an arbitrary relation $\prec$ over the elements of $S$, the following predicates define \emph{strict partial order} and \emph{strict total order}.
% \begin{align*}
%     \PartialOrder(S,\prec) \triangleq& \,(\Forall e \in S: e \not\prec e ) \land (\Forall e,e',e'' \in S: e \prec e' \prec e'' \implies e \prec e''). \\
%     %
%     \TotalOrder(S,\prec) \triangleq& \,\PartialOrder(S,\prec) \land (\Forall e,e' \in S, e \neq e': e \prec e' \lor e' \prec e).
% \end{align*}
% \end{definition}



\begin{constraint}[Total order of events] \label{cons:event-order}
The $\eo_G$ relation is a strict total order over \Events:
$$\EventTotalOrder() \triangleq \TotalOrder(\Events,\eo_G).$$
\end{constraint}

\Cref{cons:event-order} enforces that the definition of strict total order is respected by $\eo_G$.
Hence, we place ourselves in the classical (Newtonian) physics model, where events are totally ordered.
This particular assumption is critical for defining the linearizability consistency condition (see \Cref{sec:cons-cond}), which assumes a total order of events.
\jw{Note that instead of Constraint 1, we could simply define histories as sequences of events.
We use Constraint 1 to add generality in capturing models where events are not necessarily totally ordered (such as in relativistic models~\cite{GG14}). }

% \TA{cite Gilbert and Golam?}
% However, to consider relativistic scenarios, we could relax \Cref{cons:event-order} to impose only a strict partial order of events.


\begin{constraint}[Event validity] \label{cons:event-valid}
Every event must be part of exactly one op-ex:
\begin{align*}
    \EventValidity() \triangleq \Forall e \in \Events: \card{\{o=(i,r) \in \OpExes \mid e=i \lor e=r\}}=1.
\end{align*}
\end{constraint}

\begin{constraint}[Op-ex validity] \label{cons:opex-valid}
The invocation and the response events of an op-ex must be distinct, and if they are both not $\bot$, then the invocation must precede the response w.r.t. the event order:
\begin{align*}
    \OpExValidity() \triangleq \Forall (i,r) \in \OpExes: i \neq r \land (i \neq \bot \neq r \implies i \eo_G r).
\end{align*}
\end{constraint}

\begin{constraint}[Operation validity] \label{cons:ope-valid}
If an operation is a notification, then all its op-exes must be notification op-exes, otherwise, they must all be complete or pending op-exes:
\begin{align*}
    \hspace{-1.5em}\OperationValidity() \triangleq &\Forall \opp \in \Operations, \Forall o=(i,r) \in \OpExes, o.\op=\opp: \\
    & \opp.\type{=}\notif \!\Rightarrow\! (i{=}\bot \land r \!\in\! \Events)
    \land \\
    &\opp.\type{=}\normal \!\Rightarrow\! (i{\in}\Events \land r \!\in\! \Events \cup \{\bot \}).
\end{align*}
\end{constraint}
% \NN{I think the above constraint does not capture the pending op-exes or, if $\bot\in \Events$ then the last term also includes notifications.}
% \TA{Why? $\opp.\type=\normal$ only imposes that the invocation is an event, the response can be an event (complete op-ex) or $\bot$ (pending op-ex). $\bot$ is not in \Events}\NN{I think the problem stems from the fact that we do not specify what values $r$ may take. wnen $op.type = notif$ then $r\in \Events$ and when $op.type =normal$ then $r\in\Events\cup\{\bot\}$}
\JW{this maybe in the main body?}
This model does not forbid concurrent op-exes on the same process.
This way, we can consider multi-core processes that can make concurrent operation calls.
If a specifier wants to impose that op-exes on the same process behave ``in isolation'', that is, if they are concurrent, they must behave as if they happened sequentially, then he/she can apply on the history a consistency condition that ensures a per-process total order of op-exes (see \Cref{sec:cons-cond}).

% Finally, observe that we do not even impose a total order of events on the same process.
% Indeed, although it may be true in most cases, we do not need this constraint in the rest of the formalism.

==> Paragraph/Impossibility/SA-def.tex <==
% \subsection{Impossibility of Resilient Consensus Objects}
%and \texorpdfstring{$k$}{k}-Set Agreement Objects} 


% Let us first define a Consensus object as a special case of a Set-Agreement object.

\subsection{Object Definition: Set Agreement and $k$-Set Agreement}
\label{sec:SA-Definition}
\label{sec:codef}

Let us first define a Set-Agreement object $\SA$ that provides only one notification operation, $\SA.\decide_i/v$, which returns a decided value $v \in V$ to process $p_i$, where $V$ is the set of possible decisions.
Observe that we consider a very weak version of Set Agreement which has \jw{only a \decide notification, and}
no \propose operation like traditional definitions.
Indeed, proving the impossibility of this weaker version of Set Agreement (which applies also to the stronger version, where the decided value must have been previously proposed), makes our proof more general\footnote{\jw{Although, we can add a $\propose()$ operation to the set agreement object that returns nothing. The validity predicate of the $\decide()$ notification has to be adapted accordingly. This does not affect the proof.}}.

Let $\Histories$ be a distributed system's set of histories containing a Set-Agreement object $\SA$.
For every history $H=(E,\eo,O) \in \Histories$, let $H|\SA=(E|\SA,{\eo|\SA},O|\SA)$ be the subhistory containing only the events of $E$ applied to $\SA$.
Consider history $H=(E,\eo,O) \in \Histories$ with set of op-exes $O$, a relation \oo on $O$, an op-ex $o \in O|\SA$, and its context $(O_c,\oo_c) = \ctx(o,O,\oo)$.

\paragraph{Operation \decide.} If $o \equiv \SA.\decide_i/v$, then we have the following.
\begin{align*}
    \decide.\safep(o,(O_c,\oo_c)) &\triangleq (v \in V) 
    %\\
    %&
    %\land (\Nexists \SA.\decide_i/- \in O_c) 
    %\\
    %&
    \land (\Forall \SA.\decide_j/v' \in O_c: v=v'). \\
    %
    \decide.\livep(o,O,\oo) &\triangleq \Exists \SA.\decide_j/- \in O.
\end{align*}
The \safep predicate states that the values decided are in the appropriate set $V$ and that, in the context of each op-ex, 
%no process decides more than once and 
all decided values are the same. \af{Observe that we allow the same process to decide several times as long as the decided values are the same.}
%In the case of consensus, we want only one value to be decided. In order to have all values decided in the context of a $\SA.\decide_i(v)$, in the third clause a total order is very likely required ($\Serializability(H,\oo)$).
%
The \livep predicate states that some process must decide.

% \subsection{\texorpdfstring{$k$}{k}-Set Agreement}
% \label{sec:kSA}

The $k$-Set-Agreement object is the special case of Set Agreement in which at most $k$ different values are decided in each history ($1$-Set Agreement is the Consensus problem). 
In order to have a $k$-Set-Agreement object $\kSA$, we define a consistency predicate that we call $\kSetTotalOrder$ and a correctness condition that we call $\kSerializability$:
\begin{align*}
    \kSetTotalOrder(O,\oo) \triangleq &\Exists \textrm{partition~} P_1, P_2, \ldots, P_r \subseteq \Processes, r \in [1,k]: \\
    &\forall j \in [1,r], \TotalOrder(O|P_j,\oo). \\
    \kSerializability(H,\oo) \triangleq &\Legality(H,\oo) \cup \{\kSetTotalOrder(O,\oo)\}.
\end{align*}
Recall that a partition of the set $\Processes$ is a collection of disjoint subsets of the set $\Processes$, whose union is the original set.
%
Let $\Histories$ be a distributed system's set of histories containing a $k$-Set-Agreement object $\kSA$.
Then, we have the following assumption.
% \vspace{-.4em}

{\JW{TO be Polished: How do you know that the usual set agreement solvability corresponds to $kSerializability$?
Response: We can give a formal proof if convenient. The intuition is that in a history H that satisfies $kSerializability(H, \rightarrow )$ there is a k-partition of the processes so that in each set all operations are totally ordered by $\rightarrow$.
Then, from the safety property decide.S(o, ($O_c$, $\rightarrow_c$)) all the processes in a set decide the same value. 
}}

\begin{assumption}
\label{assum:kserializability}
    For every history $H=(E,\eo,O) \in \Histories$, let $H|\kSA=(E|\kSA, \eo|\kSA, O|\kSA)$ 
    be the subhistory containing only the events of $E$ applied to $\kSA$.
    Then, it holds $\Correctness(H|\kSA,\kSerializability)$.    
\end{assumption}

From the fact that \kSerializability guarantees a total order of the op-exes $O|\kSA$ of each set of processes $P_j \subseteq \Processes, j=1,\ldots, r$ on object $\kSA$, and the last clause of $\decide.\safep()$, we have the following observation.\vspace{-.4em} \\
\JW{TO be Polished: What kind of algorithms correspond to assumption 1?

Response: This assumption only says that in every history H the events of the object kSA must satisfy the correctness especification of k-set agreement, given by kSerializability: Legality as defined by decide.S and decide.L, and consistency as defined by kSetTotalOrder.}

\begin{observation}
\label{obs:k-set}
    For every history $H=(E,\eo,O) \in \Histories$, for each $j=1,\ldots, r$, all processes in $P_j$ decide the same value $v_j$ (if they decide). Hence, at most $r \leq k$ different values are decided in $\decide$ opexes.
\end{observation}

Observe that it is possible to have trivial implementations of a $k$-Set-Agreement object (in fact a Consensus object) in which all histories decide the same value $v \in V$ by simply hardcoding this in all the processes. Unfortunately, this object is not very useful.
We will impose below a non-triviality condition that guarantees that there are histories in which the $k$-Set-Agreement object decides at least $k+1$ different values. Additionally, the set of $\Histories$ must reflect the fact that the object tolerates \af{$n-1$} crash failures and the system is asynchronous.



==> Paragraph/Impossibility/SA-main.tex <==

% Main file for set agreement proof. Include this.

\section{Impossibility of Wait-free Set Agreement in Asynchronous Systems}

In this section, we use our framework to define the Set Agreement object and to provide, to the best of our knowledge, the first axiomatic impossibility proof of solving wait-free $k$-Set Agreement in an asynchronous system\footnote{Proof of the impossibility of solving Consensus in an asynchronous system with crashes is presented in \Cref{sec:consensus}.}.

% ------------- uncomment to get the previous page

\input{Paragraph/Impossibility/SA-def}

\input{Paragraph/Impossibility/SA-minusOne}

% ------------- uncomment to get the previous page


% \section{New Attempt for k-SA}

% \JW{Maybe we need new definitions of everything.}
% % ------- new attempt
% \input{Paragraph/Impossibility/SA-proof-new}


==> Paragraph/Impossibility/SA-minusOne.tex <==
\subsection{Axioms}
\label{sec:asynconcsystem}

We consider an asynchronous distributed system with $n=|\Processes|$ processes in which up to $n-1$ processes can crash. The system contains a $k$-Set-Agreement object, where $k<n$. Hence, we consider a wait-free $k$-Set-Agreement object denoted $\wfSA$.

%We consider a distributed system as described by our formalism, with a wait-free Set-Agreement object $\wfSA$.

The (potentially infinite) set $\Histories$ represents the \emph{system}.
From these histories, we will construct a (potentially infinite) set $S$ of possible states of the system.
Each \emph{state} $\state \in S$ is a (potentially infinite) set of events.
Intuitively, a state $\state$ is the collection of local states of all system processes $p_i$, represented by the totally-ordered local events $p_i$ has experienced.

\JW{Add state as a framework level concept?}
To define the set $S$, we first assign an \emph{index} to each event in a history $H=(E,\eo,O) \in \Histories$.
The index assigned to event $e \in E$ is an attribute $e.\idx$ that is the position of $e$ in the sequence of events of its process $e.\proc$.
This sequence is obtained by ordering with $\eo$ the set $E|e.\proc$.
%
Observe that the sets of events of different histories may have common events.
After adding the indices, common events with different indices are different.
For instance, the indices distinguish events in two histories in which the same process receives the same messages from the same sender but in different orders.

A special subset of $S$ is the set of \emph{complete states}, defined as 
    $\complete(S) \triangleq \{E \mid (E,\eo,O) \in \Histories \}.$
Consider now any history $H=(E,\eo,O) \in \Histories$.
We say that state $\state = E \in \complete(S) \subseteq S$ is a \emph{state extracted from $H=(E,\eo,O) \in \Histories$.}
Note that all the events in $\state$ of a process $p \in \Processes$ are totally ordered by $\eo$.
Then, we apply iteratively and exhaustively the following procedure to add more states to $S$: if $\state \in S$ is a state extracted from $H$, let $e \in \state$ be the last event (w.r.t. $\eo$),
\AF{REMOVED: "of a process $p$, "}
then $\state \setminus \{e\}$ is also a state in $S$ extracted from $H$.
Observe that this process ends when the empty state $\state=\varnothing$ is reached (which is also in $S$).
%
Intuitively, $S$ contains a state $\state$ iff there is a history $H=(E,\eo,O) \in \Histories$ such that the events in $\state$ from every process $p \in \Processes$ are a prefix of the sequence of all events from $p$ in $E$ ordered by $\eo$.

Observe that this construction of the set $S$ guarantees the following property:\vspace{-1em}

$$
    \Continuity(S) \triangleq \Forall \state \in S \setminus \varnothing, \Exists e \in \state: (\state \setminus \{e\} \in S).\vspace{-.5em}
$$

\AF{ Useful?
$$
    \Continuity(S) \triangleq \Forall \state \in S \setminus \varnothing,
    \Exists e \in \state: 
    (e.idx = |\state|e.proc|) \land (\state \setminus \{e\} \in S).\vspace{-.5em}
$$
}

\paragraph{Asynchrony Axiom.}
Moreover, any asynchronous distributed system $S$ must satisfy the following axiom.

\begin{definition}[Asynchronous distributed system axiom] \label{def:asynch-short}
The following predicate holds for the set of states $S$ in an \emph{asynchronous distributed system.}
\begin{align*}
% \Asynchrony(S) \triangleq & \Forall \state,\state' \in S: 
% (\state \cap \state' \in S) \land 
% (\procs(\state \setminus \state') \cap \procs(\state' \setminus \state) = \varnothing) \\
% &\implies (\state \cup \state' \in S),
% \\
% \Asynchrony(S) \triangleq & \Forall \state \!\in\! S: (\state \cup \{e\} \!\in S \land \state \cup \{e'\} \!\in S \land e.\proc \neq e'.\proc) \\
% &\!\!\implies\!\! (\state \cup \{e, e'\} \!\in S).
% \\
\Asynchrony(S) \triangleq & \Forall \state \!\in\! S, \forall E_1, E_2 \subseteq \Events: (\state \cup E_1 \!\in S) \land (\state \cup E_2 \!\in S) \land \\
& (\procs(E_1) \cap \procs(E_2) = \varnothing) \!\!\implies\!\! (\state \cup E_1 \cup E_2 \!\in S),
\end{align*}
where, for each set of events $E \subseteq \Events$, $\procs(E)$ is the set of processes with events in $E$.
\end{definition}

% It can shown from this definition the following general version of $\Asynchrony(S)$
% \begin{align*}
% \Asynchrony(S) \triangleq & \Forall \state \!\in\! S, \forall E', E'' \subseteq \Events: (\state \cup E' \!\in S \land \state \cup E'' \!\in S \land \\
% & \procs(E') \cap \procs(E'') = \varnothing) \!\!\implies\!\! (\state \cup E' \cup E'' \!\in S).
% \end{align*}

\af{Intuitively, \Asynchrony implies that events from different processes can be added to existing states in any order to obtain new states.}
%
We remark that our impossibility proof below is agnostic of the communication medium, as long as the medium satisfies \Asynchrony as defined above.
In \Cref{sec:examples-state-graphs}, we provide simple examples showing that systems with atomic RW Shared Memory and Reliable Broadcast satisfy \Asynchrony (thus, the impossibility proof holds), whereas Test\&Set and Total Order Reliable Broadcast do not satisfy \Asynchrony.

\AF{I propose to replace \Asynchrony with:

If there are states $\state_i \in S$  such that, $\forall e \in \state_i, e.proc = p_i$, then the state $\state = \bigcup_{i \in [1,n]} \state_i$ is also a state in $S$.
}

% \subsection{Valence}

% Attiya et al~\cite{ACR23} show that wait-free Set Agreement does not have a local-valence (FLP-style) impossibility proof.
% We show it is still possible to demonstrate impossibility using an extended valency definition associated with each pair of state and process.

% \begin{definition}[Valence function \valence]
% Given a state $E$, the \emph{valence} of $E$ over a process $p$ is a set of values given by $\valence(E, p)$ as follows.
% \begin{itemize}%[leftmargin=5mm]
%     \item If state $E \in \complete(S)$ is extracted from history $H=(E',\eo,O) \in \Histories$, $\{ v : \wfSA_p.\decide(v) \in O \} \subseteq \valence(E, p)$.
%     \item
%     $\Branching(S)$: $\Forall E \in S : \valence(E, p)=\bigcup \{ \valence(E', p): E' \in \{E \cup \{e\}: e \notin E\} \cap S \}$.
% \end{itemize}
% \end{definition}

% Then the valence of a state $E$, which is the set of values that can be decided in the histories from which $E$ is extracted, is simply the union of all processes' valences:
% $\valence(E) = \bigcup_{p\in \Processes} \valence(E, p).$

% \subsection{Resilient non-trivial Set Agreement}
% \label{sec:resSA}

\paragraph{Wait-free-Resilience Axiom.}
The following predicates describe the \minusOneResilience Axiom.

\begin{definition}[Wait-free-Resilience Set Agreement axiom] 
Given a set of states $S$ of a system with a wait-free $k$-Set-Agreement object $\wfSA$, \minusOneResilience is defined as
\label{def:n-1-Resilience}
\begin{align*}
    \minusOneResilience(S) \triangleq &\forall p_i \in \Processes :
    %\valence(\varnothing, p_i) : 
    \exists \state_i=\{e_1,...,e_r\} \in S:\\
    &(e_j.proc = p_i, \forall j \in [1,r]) \land \wfSA.\decide_i/v_i.res \in \state_i \land v_i \in V.
    %\valence(S_i, p_i) = \{v_i\}.
\end{align*}
\end{definition}

\JW{This axiom implies, as wait-freedom dictates, that each process should be able to decide by itself even if the other processes do nothing.
}

\paragraph{Non-Triviality Axiom.}
Observe that for every process $p_i$ there could be several pairs $(v_i, \state_i)$ that guarantee that $\minusOneResilience(S)$ holds. Let us denote by $F_i$ the set of values $v_i$ in these pairs. I.e., $F_i$ is the set of values that process $p_i$ can decide without any interaction with the rest of the processes. Then, for each $v \in F_i$, let $\state(v)$ denote the corresponding $\state_i$ in the corresponding pair.

\begin{definition}[Non-triviality Set Agreement axiom] 
\label{def:non-trivial}
Consider a set of states $S$ of a system with a wait-free $k$-Set-Agreement object $\wfSA$ that satisfies $\minusOneResilience(S)$. Let $F_i$ denote the set of values process $p_i$ can decide without interaction. Non triviality is defined as
\begin{align*}
%    \NonTriviality(S) &\triangleq \exists T = \{v_1, \ldots, v_n\} \subseteq F:  (\forall i \in [1,n], v_i \in F_i) \land (|T| \geq k+1).  \\
    \hspace{5em}\NonTriviality(S) &\triangleq \forall i \in [1,n], \exists v_i \in F_i:  |\{v_1, \ldots, v_n\}| \geq k+1.
\end{align*}
\end{definition}

This \NonTriviality assumption implies that without any interaction with other processes, the $n$ processes $p_i$ can decide at least $k+1$ different values $v_i$. This assumption is needed for the impossibility proof because otherwise $k$-Set Agreement can be trivially satisfied.

\begin{observation}
    If the \minusOneResilience assumption holds but the \NonTriviality assumption does not hold, allowing each process $p_i$ decide any value in $F_i$ without interaction guarantees that at most $k$ different values are decided.
\end{observation}

\subsection{Impossibility Theorem}
\label{sec:impSA}

\begin{theorem}
\label{thm:impossible-n-1}
For $k<n$, there is no asynchronous system with a wait-free $k$-Set-Agreement object \wfSA that satisfies \minusOneResilience and \NonTriviality.
\end{theorem}

\begin{proof}
\sloppy
% Let us assume such a system exists and has a set of states $S$.
\JW{Consider any algorithm $\mathcal{A}$ that implements the \wfSA object under any set of correct and faulty processes (up to $n-1$ crashes). 
Let us assume such a system exists and has a set of states $S$.
%
}
By \NonTriviality, there is a set $\{v_1, \ldots, v_n\}$ as in \Cref{def:non-trivial}.
We show that there is a history in which each process $p_i$ decides value $v_i$, for each $i\in [1,n]$. This shows that in this history at least $k+1$ different values are decided, which contradicts \Cref{obs:k-set}.

Consider the set $\{v_1, \ldots, v_n\}$ and a process $p_i$. 
Since $v_i \in F_i$, by \minusOneResilience there exist a state $\state(v_i) \in S$  such that, $\forall e \in \state(v_i), e.proc = p_i$, and $\wfSA.\decide_i/v_i.res \in \state(v_i).$
%
Then, by the \Asynchrony axiom (\Cref{def:asynch-short}), the state $\state' = \bigcup_{i \in [1,n]} \state(v_i)$ is also a state in $S$.
From \minusOneResilience, for each process $p_i$ if holds that $\wfSA.\decide_i/v_i.res \in \state'.$
%From \Branching, the valence of $p_i$ in $S'$ is identical to the valence in $S(v_i)$, i.e., $\valence(S', p_i)=\valence(S(v_i), p_i) = \{v_i\}$.
%Therefore, the valence of $S'$ is $\valence(S') = \bigcup_{i \in [1..n]} v_i = T$.
Hence let $H$ be a history from which $\state'$ can be extracted. In $H$ process $p_i$ decides value $v_i$ and hence at least $k+1$ different values are decided. This contradicts \Cref{obs:k-set}. So there is no asynchronous system with a wait-free $k$-Set Agreement object \wfSA that satisfies \minusOneResilience and \NonTriviality.
\end{proof}


==> Paragraph/Impossibility/SA-proof-new.tex <==
% Private Setup++++++
\newcommand{\LKF}{\ensuremath{\mathsf{LKF}}\xspace}
\newcommand{\Learn}{\ensuremath{\mathsf{Learn}}\xspace}
\newcommand{\Provide}{\ensuremath{\mathsf{Provide}}\xspace}

\newcommand{\SAGeneral}{\ensuremath{\mathsf{GSA}}\xspace}
% Private Setup------

\subsection{Set Agreement Object definition}

\JW{Maybe write more to connect to the state of Art later. Learn -> Immediate snapshot execution. General Structure to Shared Memory and Message Passing.}
We start by providing a general Set Agreement Structure.
Apart from decision operation, any set Agreement algorithm, in general, consists of two category operations in both the message-passing system and the shared memory system
They are the information providing operation, \verb|Provide()|, and information learning operation, \verb|Learn()| (any information must be provided first before learning.).

\paragraph{Operation \Provide.} If $o \equiv \SAGeneral.\Provide_i()$, then we have the following predicates.
\begin{align*}
    \Provide_i().proc \triangleq p_i \in \Processes
\end{align*}

\paragraph{Operation \Learn.} If $o \equiv \SAGeneral.\Learn_i(j)$, then we have the following predicates.
\begin{align*}
    &\Learn.\safep(o,(O_c,\oo_c)) \triangleq (i \in \Processes)
    %&
    \land (\Exists \SAGeneral.\Provide_j() \in O_c) \\
    &\Learn_i(j).source \triangleq p_j
\end{align*}

\JW{Assumption may need to make. $\Learn_i(j)$ only provide information to i with process j, any information come from j about k will considers as $\Learn_i(k)$}

\subsection{Decision and Local Knowledge Function}

The decision will be made deterministically based on the process's local knowledge which comes from \verb|Learn| operation.
This operation may consist of different forms, or ordering in each round.
After any round, they will either decide or abort and restart a new round.
That is, to decide is to learn.
We define such knowledge as Local Knowledge Function (LKF) below:

\paragraph{Operation \LKF.} If $o \equiv \SAGeneral.\LKF_i()$, then we have the following predicates.
\begin{align*}
    &\LKF_i() \triangleq \bigcup_{o \equiv \Learn, o.\proc=p_i} o.source \\ 
\end{align*}

Intuitively, $\LKF_i$ is the list of processes that their provided information is learned by $p_i$.


\subsection{k-set agreement}

\kSA considering a specific case of \SAGeneral.
In \kSA, there are n processes, k sets, and t faulty processes.
We denote correct process as $\delta = n - t$


\begin{lemma} 
\label{lemma:SA-SAinformationUpperBound}
Any SA algorithm that intends to learn more than n-t information violates liveness predicates.

Proof later, essential: may need to wait for a crashed process if expect more than n-t information.

\end{lemma}

\begin{definition}[Asynchronous distributed system axiom] 
% \label{def:asynch-short}
The following predicate holds for the set $S$ in an asynchronous distributed system.
\begin{align*}
\Asynchrony(S) &\triangleq \Forall E \!\in\! S: (E \cup \{e\} \!\in S \land E \cup \{e'\} \!\in S \land e.\proc \neq e'.\proc) \!\!\implies\!\! (E \cup \{e, e'\} \!\in S).
\end{align*}
\end{definition}

\subsection{Valence}

Attiya et al ~\cite{ACR23} show that $(n-1)$-set agreement does not have a local-valency (FLP-style) impossibility proof.
We show it is still possible to demonstrate impossibility using an extended valency definition associated to each pair of state and process.


\begin{definition}[Valence function \valence]
Given a state $E$, the \emph{valence} of $E$ over a process $p$ is a set of values given by $\valence(E, p)$ as follows.
\begin{itemize}%[leftmargin=5mm]
    \item If state $E \in \complete(S)$ is extracted from history $H=(E',\eo,O) \in \Histories$, $\{ v \mid \SA_p.\decide(v) \in O \} \subseteq \valence(E, p)$.
    \item
    $\Branching(S)$: $\Forall E \in S \setminus \complete(S): \valence(E, p)=\bigcup \{ \valence(E', p): E' \in \{E \cup \{e\}: e \notin E\} \cap S \}$.
\end{itemize}
\end{definition}

Then the valence function of $E$ is simply the union of all processes' valence.

$$\valence(E) = \bigcup_{p\in \Processes} \valence(E, p)$$

\subsection{Asynchronous}


NOTE: $p_i$ may learn $p_j$ without $p_j$ learns $p_i$. This follows directly from asynchronous.
Maybe a useful lemma.

\subsection{Resilient non-trivial SA}

Given a system $S$, the following predicates describe the \emph{resilient} and \emph{non-trivial} Axioms.


\begin{definition}[$(n-1)$-Resilience Set Agreement axiom] 
% \label{def:cons}
Given a set of states $S$, \minusOneResilience is defined as
\label{def:n-1-Resilience}
\begin{align*}
    \minusOneResilience(S) \triangleq &\forall p_i \in \Processes, \exists v_i \in \valence(\varnothing, p_i) : \exists KF(), |KF() \cup LKF_i| = \delta \land Val(KF()\cup LKF_i, p_i) = v_i .
\end{align*}
\end{definition}

Observe that for every process $p_i$ there could be several pairs $(v_i, LKF_i())$ that guarantee that the \minusOneResilience holds. Let us denote by $F_i$ the set of values $v_i$ in these pairs. I.e., $F_i$ is the set of values that process $p_i$ can decide without any interaction with the rest of the processes. Then, for each $v \in F_i$ let $S(v)$ denote the corresponding $S_i$ in the pair.

\begin{definition}[Non-triviality Set Agreement axiom] 
\label{def:non-trivial}
Given a set of states $S$ of a system that contains a $(n-1)$-\SA object that satisfies \minusOneResilience. Let $F_i$ denote the set of values process $p_i$ can decide without interaction, and $F=\bigcup_i F_i$. Non triviality is defined as
\begin{align*}
    \NonTriviality(S) &\triangleq \exists T = \{v_1, \ldots, v_n\} \subseteq F: |T| = n \land \forall i \in [1..n], v_i \in F_i.  
\end{align*}
\end{definition}

This \NonTriviality assumption implies that without any interaction with other processes, each process $p_i$ can decide a different value. This assumption is needed for the impossibility proof because otherwise $(n-1)$-set agreement can trivially be satisfied.

\begin{observation}
    If the \minusOneResilience assumption holds but the \NonTriviality assumption does not hold, allowing each process $p_i$ to decide any value in $F_i$ without interaction guarantees that at most $n-1$ different values are decided.
\end{observation}

\subsection{impossibility}

Hence, the possible decided value should be as large as the possible LKF.

This is the combination of $\delta$ results out of n, where each of the results may be in |V| ($|v| \geq k+1$) different situation.
